Partition Consistency: A Case Study in Modeling Systems with Weak Memory Consistency and Proving Correctness of their Implementations

Multiprocess systems, including grid systems, multiprocessors and multicore computers, incorporate a variety of specialized hardware and software mechanisms, which speed computation, but result in complex memory behavior. As a consequence, the possible outcomes of a concurrent program can be unexpected. A memory consistency model is a description of the behaviour of such a system. Abstract memory consistency models aim to capture the concrete implementations and architectures. Therefore, formal specification of the implementation or architecture is necessary, and proofs of correspondence between the abstract and the concrete models are required. This paper provides a case study of this process. We specify a new model, partition consistency, that generalizes many existing consistency models. A concrete message-passing network model is also specified. Implementations of partition consistency on this network model are then presented and proved correct. A middle level of abstraction is utilized to facilitate the proofs. All three levels of abstraction are specified using the same framework. The paper aims to illustrate a general methodology and techniques for specifying memory consistency models and proving the correctness of their implementations.

==> conclusionsWrecked.tex <==


\section{Summary, Open Questions and Future Work}
\label{concl.section}
This paper introduced partition consistency, a parameterized memory consistency model, 
from which other known models can be instantiated.
Four implementations of partition consistency that could not happen in our implementations. 
For example,
abstract memory consistency models such as P-RAM and PC-G allow a kind of cyclic causality, 
such as the computation: 

\begin{eqnarray*}
p: \ \ \opread{x}{1},  & & \opwrite{y,2}\\
q:\ \ \opread{y}{2},   & & \opwrite{x,1} 
\end{eqnarray*}
%\begin{xy}
%\xymatrix{
%p: \ \ \opread{x}{1}  \ar[r] & \opwrite{y,2}\\
%q:\ \ \opread{y}{2} \ar[r] & \opwrite{x,1} 
%}
%\end{xy}

\noindent
This computation contains a cycle. 
The first process must read the value written by the second process before writing 
but the second process must read the value written by the first process before writing.
%$p$ reads $q$'s write to $x$ before it writes $y$, and $q$ reads $p$'s write to $y$ before it writes $x$.
This problem can be overcome by adding a causality constraint to the memory consistency definitions.
Our implementations prohibit such cyclic computations. 
Hence, our implementations are stronger than the memory consistency models they implement
--- the specifications allow such computations, but our implementations do not. 
Though this computation may seem impossible in actual implementations, 
it could conceivably be possible if there is a prediction system in place. 
Our proof method could still be used with such a system.
As a second example, consider the computation:

\begin{center}
\begin{tabular}
{lccc}
$p :$ & \opwrite{x,1}, & \opread{y}{3}, & \opread{x}{1} \\
$q :$ & \opread{x}{1}, & \opwrite{x,2}, & \opwrite{y,3}
\end{tabular}
\end{center}

\noindent
This computation is possible in a Pipelined-RAM implementation that broadcasts to itself,
provided there is no guarantee that a process applies its own write before any other process applies that write. 
The first process broadcasts \opwrite{x,1} which is received and applied by the second process.
The second process then broadcasts \opwrite{x,2} and \opwrite{y,3}.
The first process receives \opwrite{x,2} before its own \opwrite{x,1} and so overwrites the 2 with a 1, 
even though \opwrite{x,1} ``caused'' \opwrite{x,2}.
This computation also could not happen in the implementations in this paper.  
This shows that our implementations are not exact, and 
that the simplest causality constraint added to the memory consistency definition is insufficient to make
it exact. 
Whether or not there is a simple strengthening of the partition consistency predicate to make our current 
implementations exact remains a question for future research.

A related issue to exactness is optimality. 
We believe that our implementations use minimal synchronization in the following sense. For every synchronization that is added by the transformation, there exists a program whose transformation would create computations that do not satisfy \PCName{} if that synchronization is removed. Confirming this intuition is beyond the scope of this paper.

Since the transformations in this paper are general, they are not optimal for all programs. Transforming individual programs may lead to more efficient implementations. Hence, another approach that we have not followed but is pursued by others (see Section \ref{related-work.section}) aims to determine for each program what synchronization is necessary and sufficient to preserve correctness on the target machine.

A different direction that could complement this research is the assessment of the performance gains of 
\PCName{} instantiations over Sequential Consistency. 
Our preliminary experiments on Westgrid's 128 node ``matrix'' cluster \cite{westgrid} are inconclusive. 
But some of these instantiations, and particularly the Weak Sequential Consistency Model, 
show a potential to outperform Sequential Consistency. 
This complementary study will be the subject of future work.


==> handshake_algorithm.tex <==

  
  \begin{codebox}

    \Procname{\func{ProtectedBlock}(\id{need},\id{doorOpen},\func{protectedAction})}

    \li $\id{need}\gets \const{true}$

    \li \While{$\neg \id{doorOpen}$} \kw{skip}

    \li \func{protectedAction}()

    \li $\id{doorOpen} \gets \const{false}$

    \li $\id{need} \gets \const{false}$

  \end{codebox}




  
  \begin{codebox}

    \Procname{\func{Guard}(\id{need},\id{doorOpen})}

    \li \If{\id{need}} 

    \li \Then  $\id{doorOpen} \gets \const{true}$

    \li \While{\id{need}} \kw{skip}

\End

  \end{codebox}




==> implementations.tex <==


\section{Implementations}
\label{implementations.section}

Our implementations transform code for a \emph{specified} model 
to code for a \emph{target} model. 
For clarity, {\sc small caps} font is used to denote specification level operations; 
{\tt Teletype} is used in  to denote target level operations.
To emphasize that a component belongs to the target level its name is sometimes
annotated with a ``hat'' as in $\widehat{\text{name}}$. 
%(\PredPC{K}{} or \PredPOB{L}{})

This section first presents the slow-write/fast-read pseudo-code for implementing \PCName{} on \POBName{},
The similar fast-write/slow-read version is in the full version of the paper \cite{cheng2009thesis}. 
Next is the pseudo-code for both the token-ring and queue implementations of the \POBName{} model on the \NWName{} model. 
%In the first implementation, $K$ is a partition of the shared variables that specifies the required agreement, 
%and the label set $L$ is constructed as a function of $K$.  
%The second implementation implements the abstract partial order broadcast specified by any label set $L$, 
%on a message passing network. 
The composition yields an implementation of any model in the abstract \PCName{} class,
including PC-G, Pipelined-RAM, WeakSC, or SC, 
where the partition of the shared variables specifies the required agreement, 
on a reliable message passing network with FIFO channels. 

\subsubsection*{Implementing \PCName{} on \POBName{}} 

Our implementation of \PCName{} using the \POBName\ model 
is a generalization of the way that Totally Ordered Broadcast is used to implement SC.
\PredPOB{L}{} enforces a similar agreement on the deliveries of updates with the same label 
as \PredPC{K}{} enforces on writes to variables within the same set in $K$.


\PCName{} models processes that interact by reading and writing globally shared variables 
that have only weak consistency guarantees.
Our task is to transform each such specified process $p$ to a target process $\widehat{p}$ 
for the \POBName\ model, 
where inter-process communication is via the partial order broadcast primitive. 
We achieve this by 1) creating a label for each partition in $K$, that is $L(K) = \{i : V_i \in K\}$; 
2) mapping each $p$  to a thread $\targ{p}.m$ in the \PredPOB{L(K)}{} model; and 3) adding to each $\widehat{p}$ a delivery thread $\targ{p}.d$. 


\begin{figure}[h]

\medskip
\noindent
\fbox{
\begin{minipage}{6.75in}
\begin{center}
\textbf{Implementing Partition Consistency on \POBName{} }
\end{center}

\noindent
\textbf{\underline{1. Transformation target variables}}\\
\begin{tabular}{ll}
%\hline
 $\id{Memory}[\widehat{p}].x$ & $\forall p\in P$, $\forall x\in V$, local replica variable, initial value is the initial value of $x$ \\
$\id{writes-processed}$   & $\forall p\in P$, local counts messages \opbcastVoid{}ed by $p$ that are also \opdeliverVoid{}ed by $p$, initially 0 \\
$\id{writes-requested}$   & $\forall p\in P$, local counts locally \opbcastVoid{}ed messages, initially 0 \\ \\
%\hline
\end{tabular}

\noindent
\textbf{\underline{2. Transforming specification threads}}\\ 
Transformation of thread $p$ to $\widehat{p}.m$ :

%\vspace*{-10pt}
\noindent
{\small 
\begin{minipage}[t]{1.60in}
\begin{codebox}
\Procname{\swimpl{K}{L(K)}{\opreadpNoReturn{x}{p}}}
\li \Return $\id{Memory}[\widehat{p}].x$
\end{codebox}
\end{minipage}
\begin{minipage}[t]{3in}
\begin{codebox}
\Procname{\swimpl{K}{L(K)}{\opwritep{x,v}{p}}}
\li $\id{writes-requested} \gets \id{writes-requested}+1$
\li \If{$\exists V_i \in K : x \in V_i$}
\li \kw{then} $\opBcast{[x,v,\widehat{p}], i}$ \kw{else} $\opBcast{[x,v,\widehat{p}], \bot}$
%\li  \Else $\opBcast{[x,v,p]}$
\li \func{WaitWritesComplete}()
\end{codebox}
\end{minipage}
\begin{minipage}[t]{2in}
\begin{codebox}
\Procname{\func{WaitWritesComplete}()}
\li \While{$\id{writes-processed} <$} 
\li \hspace*{25pt} $\id{writes-requested}$ 
\li \Do \kw{skip}
\End
\end{codebox}
\end{minipage}
}

\noindent
\textbf{\underline{3. New target threads}}\\
One new thread $\widehat{p}.d$, $\forall p \in P$ :

\noindent
{\small 
\begin{minipage}[t]{0.4\textwidth}
\begin{codebox}
\Procname{$\widehat{p}.d :$}
\li     \While  {$\myconst{TRUE}$} 
\li \Do $\func{ApplyWrite}()$ 
\End
%\end{aligned}
\end{codebox}
\end{minipage}
\begin{minipage}[t]{0.4\textwidth}
\begin{codebox}
\Procname{\func{ApplyWrite}()}
\li $\id{update}, l \gets \opDeliverNoReturn{}$
\li  $ \{ \textrm{ \id{update} has form } [x,v,source]  \}$
\li \kw{let} $[x,v,source] = \id{update}$
\li \Indent $\id{Memory}[p].x\gets v$
\li \If{$\id{source} = p $}
\li \Then $\id{writes-processed} \gets \id{writes-processed} + 1$
\End
\End
\end{codebox}
\end{minipage}
}

\end{minipage}
}
\medskip

\caption{Implementing \PCName{} on \POBName{} model }
\end{figure}


The main thread, $\widehat{p}.m$, is identical to $p$ except that each \opreadVoid{} 
and \opwriteVoid{} to a shared variable is replaced by a subroutine call. 
The transformation of a \opreadVoid{} simply returns the value stored in $\widehat{p}$'s local memory. 
The transformation of a \opwriteVoid{} creates a \opBcastVoid{} operation to be \opDeliverVoid{}ed to each target process.
It has a label corresponding to the partition of the variable being written, if this partition exists.



The delivery thread, $\widehat{p}.d$, manages the \opDeliverVoid{} operations 
and maintains synchronization with $\widehat{p}.m$ via locally shared variables.
It indefinitely applies updates to the local memory it shares with $\widehat{p}.m$.
The procedure \func{WaitWritesComplete} causes $\widehat{p}.m$ to wait 
until $\widehat{p}.d$ has applied all the \opwriteVoid{}s previously broadcast by $\widehat{p}.m$. 


Under the $\swimpl{K}{L(K)}{}$ transformation,
each process has at most one outstanding local write,
since every write must be applied locally before the subroutine completes.
Every write contains a wait, making these writes ``slow''. 
An alternative is to move the \func{WaitWritesComplete} call from the end of the \opwriteVoid{} to the beginning of the \opreadVoid{}. 
This gives us a fast-write/slow-read (\fwimpl{K}{L(K)}{}) implementation described in the full version \cite{cheng2009thesis}. 


\subsubsection*{Implementing \POBName{} on \NWName{} using tokens \tokenimpl{L}{}} 

The \POBName{} model is very similar to the \NWName{} model: we need only specify how to implement $\opbcastVoid{}$ and \opdeliverVoid\ by \opSendVoid{}ing
and \opRecvVoid{}ing messages.
The operations \opreadVoid\ and \opwriteVoid{}  are simply mapped through with an identity transformation.
The processes in \Processes\ are numbered starting at 0, 
and organized into a virtual ring such that $ \func{next}(p) = (p + 1)\; \kw{mod}\; \abs{\Processes} $. 
A token is created for each label $l\in L$, and for each token, a thread is created on each process to manage it.

To broadcast an update with a $\bot$ label, we \opSendVoid{} it to every other process since these updates only require FIFO ordering.
Updates with a non-$\bot$ label need to maintain a per-label total order.  For such updates, we acquire the label's token, then \opSendVoid{} the update to every other process, and wait for acknowledgments before continuing.


\begin{figure}[!ht]
\medskip
\noindent
\fbox{
\begin{minipage}{6.75in}
\begin{center}
\textbf{Using Tokens to Implement \POBName{} on \NWName{}}
\end{center}

\noindent
\textbf{\underline{1. Transformation target variables}}\\
\begin{tabular}{ll}
 $\id{need-token}_l$ & for each $l\in L$ and $p\in P$,  handshake variable \\
 $\id{door}_l$ & for each $l\in L$ and $p\in P$,  handshake variable \\
$\widehat{x}$ & for each $x \in V$,   identity transform \\
\end{tabular}

\noindent
\textbf{\underline{2. Transforming specification threads}}\\ 
Transformation of thread $p.m$ to $\widehat{p}.m$ and $p.d$ to $\widehat{p}.d$ :

%\vspace*{-10pt}
\noindent
{\small 
\begin{minipage}[t]{3in}
  \begin{codebox}

    \Procname{$\tokenimpl{L}{\opbcast{ u , l }}$}
    \li \If{$l \ne \bot $}
    \li \Then  $\func{ProtectedBcast}(\id{need-token}_l, \id{door}_l , u , l )$  	
    \li \Else $\func{bcastop}(u,l)$
  \End
  \end{codebox}
\end{minipage}
\begin{minipage}[t]{2in}
  \begin{codebox}
    \Procname{$\tokenimpl{L}{\opdeliverNoReturn{}}$}
    \li $\codeRecvPattern{q,p,[\myconst{MESSAGE} , u , l ]}$
    \li \If $l \ne \bot$
    \li \Then $\opSend{p,q, [\myconst{ACK}]}$
\End
\li \Return $u , l$ 
  \end{codebox}
\end{minipage}
\begin{minipage}[t]{1.55in}  
\begin{codebox}
\Procname{$\tokenimpl{L}{\opreadNoReturn{x}}$}
\li \Return $\widehat{x}$
\end{codebox}

\begin{codebox}
\Procname{$\tokenimpl{L}{\opwrite{x,v}}$}
\li $\widehat{x} \gets v$
\end{codebox}
\end{minipage}
}

\noindent
{
\begin{minipage}[h]{0.4\textwidth}
  \begin{codebox}

    \Procname{\func{ProtectedBcast}(\id{need},\id{doorOpen},$m$, $l$ )}

    \li $\id{need}\gets \myconst{TRUE}$

    \li \While{$\neg \id{doorOpen}$} \kw{skip}

    \li $\func{bcastop}( u , l )$

    \li $\id{doorOpen} \gets \myconst{FALSE}$

    \li $\id{need} \gets \myconst{FALSE}$

  \end{codebox}
\end{minipage}
\begin{minipage}[h]{0.4\textwidth}
  \begin{codebox}
    \Procname{\func{bcastop}($u , l $)} 
%\li $\{\textrm{Broadcast}\}$
    \li \kw{forall} $q \in P $ 
    \li \Do $\opSend{p , q , [ \myconst{MESSAGE} , u , l]}$
\End
\li \If {$ l \ne \bot $ }
\li $\{\textrm{Wait for acknowledgment}\}$
\li \Then \kw{forall} $q \in P $ 
\li \Do $\codeRecvPattern{q , p , [\myconst{ACK}]}$
  \End
  \End
  \end{codebox}
\end{minipage}
}

\noindent
\textbf{\underline{3. New target threads}}\\
One new token thread $\widehat{p}.\func{TokenThread}_l$, $\forall p \in P , l \in L$ :

\noindent
{\small 
 \begin{minipage}[t]{4.0in}
            \begin{codebox}
           \Procname{$\targ{p}.\func{TokenThread}_{l}:$}
              \li \If{$\targ{p} = 0 $}
              \li \Then $\opSend{\targ{p},\func{next}(\targ{p}), [\myconst{TOKEN}, \myconst{BCASTGROUPTOKEN}_l]}$
            \End
            \li \kw{loop}
            \li \Do $\func{PassToken}_{\targ{p}}(l)$
          \End
            \end{codebox}
        \end{minipage}
\begin{minipage}[t]{1.5in}
  \begin{codebox}
    \Procname{$\func{next}(\widehat{p})$}
    \li \Return $(\widehat{p} + 1) \; \kw{mod} \; \left|\widehat{P}\right|$
  \end{codebox}
\end{minipage}

} 
\begin{minipage}[t]{0.5\textwidth}
  \begin{codebox}         
    \Procname{$\func{PassToken}_p(l)$}
    \li $\codeRecvPattern{q,p,[\myconst{TOKEN}, \myconst{BCASTGROUPTOKEN}_l]}$ 
    \li $\func{Guard}(\id{need-token}_l,\id{door}_l)$
    \li $\opSend{p,\func{next}(p), [\myconst{TOKEN}, \myconst{BCASTGROUPTOKEN}_l]}$
  \end{codebox}
\end{minipage}
\begin{minipage}[t]{0.4\textwidth}
  \begin{codebox}

    \Procname{\func{Guard}(\id{need},\id{doorOpen})}

    \li \If{\id{need}} 

    \li \Then  $\id{doorOpen} \gets \myconst{TRUE}$

    \li \While{\id{need}} \kw{skip}

\End

  \end{codebox}
\end{minipage}
\end{minipage}
}
\medskip

\caption{Token implementation of \POBName{}}
\end{figure}

Each call to \func{PassToken} manages one acquisition and subsequent release of a token.
It calls the \func{Guard} subroutine each time it acquires a token.
The \func{Guard} returns only after handshaking with \func{ProtectedBcast}
to determine that the token is no longer needed and can be released. 
%Pattern matching is used to ensure token threads receive only the messages that are related to their token.
$\codeRecvPattern{pattern}$ is pseudo-code that blocks until a message matching 
$pattern$ is received and stored in the appropriate pattern variables.



The transformation of \opbcastVoid{} acquires the appropriate token to broadcast 
a labeled message by synchronizing with its token thread.
The broadcast of a labeled message further requires that all processes deliver the message before the token is released.
To ensure this, the implementation of \opbcastVoid{} waits for acknowledgments from all the processes before completing.
%This requires that the deliver operations of a process are performed on a separate thread from the bcast operations.
%A separate deliver thread is used to receive all broadcasts and send acknowledgments, for labeled messages.
To avoid deadlock this transformation requires that \opbcastVoid{}s and \opdeliverVoid{}s are invoked by separate threads.


Unlabeled messages are broadcast without acquiring a token. 

%\vspace*{-10pt}
%The parameter $L$ of the transform $\tokenimpl{L}{}$ is needed because a token is created for each label.
%To clarify the presentation, we will often drop the parameter and just write $\tokenimpl{L}{}$, 
%as $L$ will be provided by the specification $\PredPOB{L}{}$.


\subsubsection*{Implementing \POBName{} on \NWName{} using timestamps \tsimpl{L}{}}
\label{queue-algorithm}
Instead of strongly ordering the deliveries in time using tokens, the \tsimpl{}{} implementation uses timestamps to enforce an agreement on the order of deliveries.
This implementation generalizes Attiya and Welch's timestamp total order broadcast implementation \cite{attiya2004dcf}.

The implementation uses
priority queues, but since each one is only accessed by one thread, 
they can be constructed out of variables.
One queue is created for each message label and one for unlabeled messages.
Priority queues ensure that when a message is dequeued, it has the least timestamp out of the remaining messages in the same queue.
If we further ensure that all messages with a smaller or equal timestamp have been received and \opEnqueueVoid{}'d before \opDequeueVoid{}ing a message, then all processes will deliver messages with the same label in the same order.
Because messages are spread across the multiple priority queues, FIFO delivery order is not automatically enforced.
To satisfy FIFO delivery order, we require that a message is only delivered by a process if it has the next counter value after the counter of the last delivered message from that source.



\begin{figure}[!ht]
\medskip
\noindent
\fbox{
\begin{minipage}{6.75in}
\begin{center}
\textbf{Using Timestamps to Implement \POBName{} on \NWName{}}
\end{center}

\noindent
\textbf{\underline{1. Transformation target variables}}\\
\begin{tabular}{ll}

 \id{counter} & for each $p\in P$,  local  array of last delivered counter value for each process, initially all 0\\
\id{T} & for each $p\in P$, local array of last received timestamp value for each process, initially all 0\\
$\id{queue}_l$ & for each $l\in L$ and $p\in P$   local priority queue for messages labeled $l$, initially empty \\
 \id{fifo} & for each $p\in P$,  local array of queues for unlabeled messages, one queue for each process,\\ & initially all empty\\
$\widehat{x}$ & for each $x \in V$,  $\widehat{x}$ identity transform of $x$ \\
\end{tabular}

\noindent
\textbf{\underline{2. Transforming specification threads}}\\ 
Transformation of thread $p.m$ to $\widehat{p}.m$ and $p.d$ to $\widehat{p}.d$ :

%\vspace*{-10pt}
\noindent
{\small
\begin{minipage}[t]{0.3\textwidth}
\begin{codebox}
\Procname{$\tsimpl{L}{\opreadNoReturn{x}}$}
\li \Return $\widehat{x}$
\end{codebox}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
\begin{codebox}
\Procname{$\tsimpl{L}{\opwrite{x,v}}$}
\li $\widehat{x} \gets v$
\end{codebox}
\end{minipage}
\begin{minipage}[t]{0.6\textwidth}
  \begin{codebox}
    \Procname{$\tsimpl{L}{\opbcast{\id{update} , l}}$}
    \li  $\opSend{\widehat{p},\widehat{p}, [\blankfrac{\const{local-broadcast-request}, }{ \id{update} , l}]} $
  \end{codebox}
\end{minipage}
\begin{minipage}[t]{0.4\textwidth}
  \begin{codebox}

    \Procname{$\tsimpl{L}{\opdeliverNoReturn{}}$}
    \zi $\Set{\quad l \textrm{ can be } \bot \quad}$
    \li \While{$(\neg \exists l\in L : \func{CanExtract}(queue_l))$}
    \li $\wedge (\neg \exists \widehat{p} \in \widehat{P} : \func{CanDequeue}(\id{fifo}[\widehat{p}]))$
    \li \Do \func{HandleMessage()}
\End
\li \kw{case} (\kw{choose} $ (\const{L} l : \func{CanExtract}(queue_l))$
\li $| (\const{U} \widehat{p} : \func{CanDequeue}(\id{fifo}[\widehat{p}]))$)
\li \kw{of}
\li $(\const{L} l)$ \kw{then}  $m \gets \opDequeueNoReturn{queue_l}$
\li $(\const{U} \widehat{p})$ \kw{then}  $m \gets \opFIFODequeueNoReturn{\id{fifo}[\widehat{p}]}$
\li $counter[m.src] \gets m.counter$
\li \Return $m.\id{update} , m.l$
  \end{codebox}
\end{minipage}
\begin{minipage}[t]{3.625in}
  \begin{codebox}

    \Procname{$\func{HandleMessage}_p()$}

    \li $\widehat{s}, \widehat{p}, \id{message}\gets \opRecvNoReturn{}$

    \li \kw{case} \id{message} \kw{of}:
    \li $[\const{local-broadcast-request},\id{update}, l]$
    \li \Then $T[\widehat{p}] \gets T[\widehat{p}]+1$ 
    \li  $\id{local-counter} \gets \id{local-counter} + 1$
    \li  $\id{prepmessage} \gets [\blankfrac{ \const{ord-msg} , \id{update} , l }{ T[p], \id{local-counter} , \widehat{p} }]$
    \li  $\func{ProcessMessage}(\id{prepmessage}, l)$
    \li  $\func{FifoBroadcast}(\id{prepmessage})$
\End
\li  $[\const{ts-update}, \id{timestamp}, \widehat{q}]$
\li \Then  $T[\widehat{q}]\gets \id{timestamp}$
\End
\li $[ \const{ord-msg} , \id{update}, l, \id{timestamp} , \id{counter} , \widehat{q} ]$
\li \Then $T[\widehat{q}] \gets \id{timestamp}$
\li \func{ProcessMessage}(\id{message},l)
\li \If{$timestamp > T[p]$} \label{queue-pob-update-condition}
\li \Then $T[\widehat{p}] \gets \id{timestamp}$
\li $\func{FifoBroadcast}([\const{ts-update} , T[\widehat{p}] , \widehat{p}])$
\End

  \End
  \end{codebox}
\end{minipage}
}

\noindent
\begin{minipage}[t]{3.625in}

\end{minipage}
\begin{minipage}[t]{3in}


\end{minipage}

\noindent
\textbf{\underline{3. New target threads}}\\
No new target threads for this implementation.

\end{minipage}
}
\medskip

\caption{Timestamp implementation of \POBName{}}
\end{figure}

\begin{figure}[!ht]
\fbox{
\noindent
\begin{minipage}{3.5in}
  
  \begin{codebox}
    \Procname{$\func{CanExtract}(queue)$}
    \li \If{$\opIsemptyNoReturn{queue}$}
    \li \Then \Return \const{false}
    \li \Else $m \gets \opPeekminNoReturn{queue}$
    \li \Return $(m.counter = counter[m.src] + 1)$
    \zi  \quad $\wedge (\forall \widehat{q}\in \widehat{\Processes{}} : m.ts < T[\widehat{q}]) $
  \End
  \end{codebox}
\begin{codebox}
\Procname{$\func{CanDequeue}(\id{fifo-queue})$}
\li \If{ \opFIFOIsEmptyNoReturn{\id{fifo-queue}} }
\li \Then \Return \mfalse{}
\li \Else $m \gets \opFIFOPeekHeadNoReturn{\id{fifo-queue}} $ 
    \li \Return $(m.counter = counter[m.src] + 1)$
\End
\end{codebox}
\end{minipage}
\begin{minipage}{3.25in}
   \begin{codebox}
    \Procname{$\func{ProcessMessage}(\id{message}, l)$}
    \li \If{$l \ne \bot$}
    \li \Then  $\opEnqueue{\id{queue}_{l}, \id{message}}$
    \li \Else  $\opFIFOEnqueue{\id{fifo}[\id{message}.\id{src}], \id{message}}$
  \End
  \end{codebox}

\begin{codebox}
\Procname{$\func{FifoBroadcast}(\id{message})$}
\li \For $\widehat{q} \in \widehat{P} \setminus \{\widehat{p}\}$
\li \Do \opSend{ \widehat{p} , \widehat{q} , \id{message} }
\End
\end{codebox} 
\end{minipage}
}
\caption{Auxiliary functions for Timestamp implementation}
\end{figure}

This implementation requires that for each process, at most one thread performs \opdeliverVoid{}.
The first piece is the transformation of \opbcastVoid{}.
Since the actual broadcast requires modifying the priority queue, we pass this responsibility on to the transformation of the \opdeliverVoid{} operation to avoid race conditions and more complicated synchronization.

The \opdeliverVoid{} transformation does the heavy lifting in this implementation.
It drives the processing of messages by calling \func{HandleMessage} when it cannot return anything.
The \func{HandleMessage} function handles all the background maintenance work, sending timestamp updates, 
modifying the timestamp and counter arrays, and queueing messages.

Messages contain labels indicating which queue they belong to, as well as other fields needed for the protocol.
Unlabeled messages are queued in the special queue $\id{queue}_{\bot}$.
The notation $m.ts$ denotes the $\id{timestamp}$ field of a $\const{ord-msg}$ or
$\const{ts-update}$ message $m$.
The notation $m.src$ denotes the message source field of an $\const{ord-msg}$.
The notation $m.counter$ denotes the program counter field of an $\const{ord-msg}$.

The implementation of \func{FifoBroadcast} relies on the underlying model to provide FIFO properties.
Reads and writes are mapped through with an identity transform.
$\widehat{x}$ is used to emphasize that the model has changed. 


The parameter $L$ of the transform $\tsimpl{L}{}$ is needed since a priority queue is created for each label in $L$.
To clarify the presentation, we will often drop the parameter and just write $\tsimpl{}{}$, as $L$ will be provided by the specification $\PredPOB{L}{}$.



==> proofs.tex <==


\section{Proofs of Correctness of the Implementations}
\label{proofs.section}

\subsection{Proof structure and setup}
\label{proofs.structure.section}

Section \ref{implementations.section} presented transformations of a specified multiprogram into a target multiprogram.
To prove correctness, we must show the possible computations of these two multiprograms that can arise from their respective
memory consistency model, have the same ``outcome''.  
We make this precise as follows.
Let \transform{\Processes} denote a transformation of multiprogram \Processes.
The possible computations of multiprogram \Processes\ (respectively, \transform{\Processes})
on the specified (respectively, target) memory consistent model \memCon (respectively, \MemCon) 
is the set \FiltermemConVoid{{\Processes}} 
(respectively, \FilterMemConVoid{{\transform{\Processes}}}).
But \transform{\Processes} transforms specified operation invocations that require a response 
into subroutines that return a response.  
So these returned responses can be used to \emph{interpret} each computation in
\FilterMemConVoid{{\transform{\Processes}}} as a computation of
\Processes.
We need to show that each such interpreted computation could have arisen in the specified model.
That is, we must show that 
the interpretation of any computation in \FilterMemConVoid{{\transform{\Processes}}} is in 
\FiltermemConVoid{\Processes}.
If this is satisfied for any \Processes, we say that \transform{\Processes} \emph{correctly implements}
\memCon{} on \MemCon{}.
Figure \ref{correctnessPlan.figure} (at the end of this paper) depicts this proof obligation for the transformations in Section \ref{implementations.section}. 


\begin{figure}[p]

\begin{xy}
\xymatrix{
\ComputationSet{P} \ar[d]_{\swimpl{K}{L(K)}{P}} &  \ar@{--}[l]_{\supseteq} \FilterMemCon{\PC{K}}{P} &  \ar@{--}[l] _(0.2){\textnormal{show } \supseteq} I \\
 & & \\
  \ComputationSet{\swimpl{K}{L(K)}{P}} \ar[d]_{\tsimpl{L(K)}{}} &  \ar@{--}[l]_{\supseteq} \FilterMemCon{\PredPOB{L}{}}{\swimpl{K}{L(K)}{P}} \ar @{--}[ru]_{\textnormal{interpret}}&   \ar@{--}[l]_(0.2){\textnormal{show } \supseteq} \widehat{I} \\
& & \\
 \ComputationSet{ \tsimpl{L}{ \swimpl{K}{L(K)}{P} } } &   \ar@{--}[l]_(0.6){\supseteq} \FilterMemCon{\PredNW{}}{ \tsimpl{L}{ \swimpl{K}{L(K)}{P} }}  \ar @{--}[ru]_{\textnormal{interpret}}& & \\
}
\end{xy}

\caption{Proof obligation for establishing correctness of transformations}
\label{correctnessPlan.figure}
\end{figure}


We show that a computation satisfies a model by constructing a collection of orders that jointly satisfy the model's constraints.
We call collections of orders showing that a computation satisfies a memory consistency model, \emph{witness orders} to that consistency model.

\subsection{Proof method:}
%\subheader{Outline of memory consistency proofs:}
The proofs, including all four in the full paper, have the following structure:\\
\fbox{\bf{}Assume:}
 $\widehat{C} \in  \FilterMemConVoid{{\transform{\Processes}}}$.
 Let $C\in \ComputationSet{P}$ be the interpretation of $\widehat{C}$. \\
\fbox{\bf{}Build:}
Choose some collection of \emph{witness orders} $\widehat{A}$ that satisfy $\MemCon{}[\widehat{C}]$.
Use $\widehat{A}$ to construct a corresponding collection of orders $A$ for $C$. \\
\fbox{\bf{}Verify:}
Show that the collection $A$ are witness orders to $\memCon{}[C]$. 

This method is similar in concept to reduction proofs in complexity theory and simulation proofs for equivalence of systems.
The transformation directly produces target level operations from specification level ones.
However, the actual target level operations that are most important for the execution of the specification level operation will depend on the interaction between concurrent processes and operations at the target level.
The {\bf{Build}} step involves finding these key target level operations and mapping them back to the specification level.
Implementations that abstract away more intricate interactions at the target level will often require more subtle mappings than the direct one provided by the transformation.


In this paper, we consider only \emph{finite} computations, and completed computations produced by transformations of these computations.
For long-lived computations, we would need to allow only a prefix of the required messages or updates to be \oprecvVoid{}'d or \opdeliverVoid{}'d, order operations not seen by certain processes in their views and handle these changes in the proofs.


We prove the required lemmas assuming the computations, orders and constructed orders of the \specialsubheaderinline{Assume} and \specialsubheaderinline{Build} steps of the theorem.
In developing these proofs, we found that a diagram format helped uncover many underlying assumptions and errors in the proofs.
This diagram format also allowed us to quickly work out proofs on a whiteboard.  
Before presenting the lemmas we digress to describe the proof diagram format.

\subsection{Proof diagrams}
\label{proof-diagrams}

Edges in the diagram represent boolean expressions and the
diagram is interpreted as the conjunction of these expressions.
The basic building blocks are:

\noindent\begin{tabular}{p{2.625in}p{3.625in}}
$
\xymatrix{
a \ar@{=}[r] & b
}
$ asserts that $a=b$. 

$
\xymatrix{
a \ar[r]^{L} & b
}
$
asserts that $a\orderArrow{L}b$.


$\xymatrix{
a \ar@{--}[r]^R & b 
}$ asserts that $a$ is related to $b$ by a relation $R$.

&

$\xymatrix{
a \ar[rr]^{L}& \ar@{=>}[d] & b \\
c \ar[rr]_{M}& & d
}
$ asserts that $(a \orderArrow{L} b) \implies (c\orderArrow{M} d)$.
\end{tabular}

For sets $A$ and $B$, using notation similar to Lamport's system executions \cite{lam86b} we have:

\noindent
\begin{tabular}{p{3.125in}p{3.125in}}
$
\xymatrix{
A \ar[r]^{L} & B
}
$
asserts that $\forall a\in A, b \in B : a\orderArrow{L}b$.
&
$
\xymatrix{
A \ar@{|-->}[r]^{L} & B
}
$
asserts that $\exists b \in B :\forall a\in A : a\orderArrow{L}b$.
\\
$
\xymatrix{
A \ar@{-->|}[r]^{L} & B
}
$
asserts that $\exists a\in A : \forall b \in B : a\orderArrow{L}b$.
&
$
\xymatrix{
A \ar@{-(}[r] & B
}
$ asserts that $A\subseteq B$.
\end{tabular}

Multiple edges between two nodes denote the disjunction of the corresponding assertions.
So $\xymatrix{a \ar@/_/[r]^{{\scriptscriptstyle D}} \ar@/^/[r]^{{\scriptscriptstyle E}} & b}$ asserts
that $a\orderArrow{D} b$ or $a\orderArrow{E} b$.
%In order to assert that $a \orderArrow{D} b$ and $a\orderArrow{E} b$ we would use:
%
%\begin{xy} 
%\xymatrix{
%a \ar[r]_{D} &  b \\
%a \ar@{=}[u] \ar[r]_{E} & b \ar@{=}[u] \\
%}
%\end{xy}
%
The direction of the edge will indicate which way it should be read.
For example $
\xymatrix{
a \ar[r]_L & b
}
$ and
 $
\xymatrix{
b & a \ar[l]^L
}
$ are equivalent.


\subsection{Correctness of the \swimpl{K}{L(K)}{} and \fwimpl{K}{L(K)}{} implementations}

The proofs of \fwimpl{}{}{} and \swimpl{}{}{} are very similar, they only differ in one step.
This step can be treated generically, so we present one proof for both implementations.
Let $\wimpl{K}{L(K)}{}$ refer to either implementation.

Let $\Processes{}$ be a program compatible with the $\PredPC{K}{}$.
This means that $\Processes{}$ must be a single threaded program that only operates on read/write variables.

\begin{theorem}
\label{wrtrans-correctness-theorem}
\wimpl{K}{L(K)}{} correctly implements \PredPC{K}{} on \PredPOB{L(K)}{} for any $K$.
\end{theorem}

\begin{specialproof}


\specialsubheader{Assume:}
Let $\widehat{C}$ be a computation in $\ComputationSet{\wimpl{K}{L(K)}{P}, \PredPOB{L(K)}{}}$ and let $C$ be a computation in $\ComputationSet{P}$  such that $\widehat{C}$ is an interpretation of $C$.
Let $\widehat{O}$ denote the set of operations $O_{\widehat{C}}$.

\specialsubheader{Build:}
We construct orders $\MapSet{(O_{C}|p\cup O_{C}|\cutwrites,\orderArrow{L_p}) : p\in P: }$ to satisfy the partial order and agreement constraints of $\PredPC{K}{}$. \\
Let  $\MapSet{(O_{\widehat{C}}|\widehat{p}, \relLinearp{} ): p \in \wimpl{K}{L(K)}{P} : }$ be witness orders to $\PredPOB{L(K)}{\widehat{C}}$.

For a total order $(O,\orderArrow{X})$, we denote its induced sequence by $X$.
Construct  $\MapSet{(O_{C}|p\cup O_{C}|\cutwrites,\orderArrow{L_p}) : p\in P: }$  as follows:

\begin{enumerate}
\item For each operation $o$ on a ``local replica'' variable we associate it with a specification level operation by defining a relation $\constructArrow$
  \begin{enumerate}
  \item 
    $\opRead{\id{Memory}[p].x}{v}$ by the transformation, this operation must have come from the transformation of a specification level  $\opread{x}{v}\in O|p$.  Associate it with this specification level operation by letting: $$\opRead{\id{Memory}[p].x}{v}\constructArrow \opread{x}{v}$$
  \item
    Every $\opWrite{\id{Memory}[p].x,v}$ must have a $o_d = \opdeliver{[\const{write},x,v]}$ in the same $\func{ApplyWrite}()$ call.
    This deliver operation $o_d$ must have a corresponding $\opbcast{m}$, which can only have occurred in the transformation of some high level write  $\wimpl{K}{L(K)}{\opwrite{x,v}}$. Associate the original operation with this specification level one by letting:
 $$\opWrite{\id{Memory}[p].x, v}\constructArrow \opwrite{x, v}$$

  \end{enumerate}
\item Build the sequence $Short(\seqLinearp)$ from the sequence \seqLinearp{} by removing all of the operations of the broadcast object, and the variables \id{writes-processed} and \id{writes-requested}.  
This leaves only the operations on the ``local replica'' variables.
\item Build the sequence $\seqlinearp$ as follows: every operation in $Short(\seqLinearp{})$  is a local memory read or write on a replica so we replace them with their associated high level operations.  This sequence induces the required total order.
\end{enumerate}

Specification level \opReadVoid{}s are transformed to target level local replica \opreadVoid{}s, so for reads $\constructArrow{}$ is the inverse of the transformation.
Specification level \opWriteVoid{}s on the other hand are transformed to a \opbcastVoid{} of the \opWriteVoid{} data.
The actual \opbcastVoid{} is not as key to the mapping as the local replica \opwriteVoid{}s performed when the updates are \opdeliverVoid{}ed.

The operations that are deleted are not important for the mapping, but they are important for enforcing the ordering of operations.
This implementation has a clean separation between the \opbcast{} primitives and shared variable handshaking that deal specifically with ordering, and the local operations on the replicas that deal with the semantics of the specification level operations.

The constructed sequences $\MapSet{\;L_p : p\in P: \;}$ induce corresponding total orders \\ $\MapSet{(O|p\cup O|\cutwrites, \orderArrow{L_p}) : p\in P : \;}$.

\specialsubheader{Verify:} 
We prove that the constructed orders $\orderArrow{\seqlinearp{}}$ are witnesses to  $\PredPC{K}{C}$.

To show this, we directly prove that the total orders constructed in the previous section, $\MapSet{(O|p\cup O|\cutwrites, \orderArrow{L_p}) : p\in P : \;}$, satisfy each of the properties in Definition \ref{general-mcm-defn}.
These total orders are valid by the way that they were constructed from the valid witness total orders $\MapSet{\;\orderArrow{\seqLinearp}: \widehat{p}\in \widehat{P} \:\;}$.
Removing all operations related to specific objects preserves validity when forming $\func{Short}(\seqLinearp)$.
Replacing reads and writes with corresponding reads and writes also preserves validity.

 The remaining $\PredPOB{L(K)}{}$ constraint are satisfied owing to the following Lemmas:


\begin{tabular}{|l | r|}
\hline
Constraint & Lemma\\
\hline
$ \Pred{Extends}[\orderArrow{L_p}, \orderArrow{\programOrder} , O|p \cup O|\cutwrites ]$ & Lemma \ref{top-middle-prog-extend} \\
$ \forall p,q \in P, i\in [1,k] :  \Pred{Agree}[\orderArrow{L_p}, \orderArrow{L_q}, O|\cutwritesgroup{S_i}] $ &  Lemma \ref{top-middle-group-ordering} \\
\hline
\end{tabular}\medskip
 
Therefore $\PredPC{K}{C}$ as required.
\end{specialproof}

%% For the following lemmas, let $\widehat{C}\in \computationSet{\wimpl{K}{L(K)}{P},\wimpl{K}{L(K)}{J}, }$ and let $C$ such that $\widehat{C} \modelArrow{\func{WRtrans}^{*-1}} C$ as in the \specialsubheaderinline{Assume} step of Theorem \cite{wrtrans-correctness-theorem}.
%% And let $\MapSet{\orderArrow{\seqLinearp{}} : p\in \Processes:}$ be constructed as in the \specialsubheaderinline{Build} step of Theorem \cite{wrtrans-correctness-theorem}.

Let $\widehat{C}\in \computationSet{\wimpl{K}{L(K)}{P},\wimpl{K}{L(K)}{J}, \PredPOB{L(K)}{}}$.
Let $C$ be such that  $\widehat{C}$ is an interpretation of $C$.
This matches the \specialsubheaderinline{Assume} step of Theorem \ref{wrtrans-correctness-theorem}.

Let $\MapSet{(O_{\widehat{C}}|\widehat{p}, \relLinearp{} ): p \in \wimpl{K}{L(K)}{P} : }$
 be witness orders that satisfy  $\PredPOB{L(K)}{\widehat{C}}$. 
Construct  $\MapSet{\orderArrow{\seqlinearp{}} : p\in \Processes:}$  
based on the chosen witness orders as in the \specialsubheaderinline{Build} step of Theorem  \ref{wrtrans-correctness-theorem}. 

\begin{lemma}
\label{top-middle-prog-extend}
  $\forall p\in P :\Pred{Extends}[ \orderArrow{L_p}, \orderArrow{\programOrder}, O|p \cup O|\cutwrites]$
\end{lemma}

\begin{specialproof}
  Let $o_1,o_2$ be operations in $O|p \cup O|\cutwrites$ so that $o_1\orderArrow{\programOrder} o_2$.
Since they are ordered by program order, they must have been invoked by the same process, so $proc(o_1)=proc(o_2)=q$ for some $q$.
\PredPC{K}{} only has read/write variable objects, so there are four cases for $o_1,o_2$:

\subheader{Case 1: read, read} 
Then $o_1=\opread{x}{v}$ and $o_2=\opread{y}{w}$

We have $ p = q $ and $ \wimpl{K}{L(K)}{o_1} \orderArrow{\ProgramOrder} \wimpl{K}{L(K)}{o_2} \implies o_1  \rellinearp{} o_2$ since the reads are directly translated, they remain in program order.

\subheader{Case 2: read, write} 
Then $o_1=\opread{x}{v}$ and $o_2=\opwrite{y,w}$:

We have $ p = q $ and $ \wimpl{K}{L(K)}{o_1} \orderArrow{\ProgramOrder} \wimpl{K}{L(K)}{o_2} $ which implies 
% $$ \opRead{x}{v}  \relLinearp{} \opBcast{o_2}  \relLinearp{} \opDeliver{o_2}  \relLinearp{} \opWrite{Memory[p].x,v} $$ 
 \[
\xymatrix{ 
\opread{x}{v} \ar@{--}[d]_{\wimpl{K}{L(K)}{}} \ar[r]^{\programOrder} & \opwrite{y,w} \ar@{--}[d]_{\wimpl{K}{L(K)}{}} \\ 
\wimpl{K}{L(K)}{o_1} \ar@{)-}[d] \ar[r]^{\ProgramOrder} & \wimpl{K}{L(K)}{o_2} \ar@{)-}[d]& & \\
\opRead{x}{v} \ar[r]_{\seqLinearp} \ar@{--}[d]_{\id{construct}} & \opBcast{o_2}  \ar[r]_{\seqLinearp}^{1.} & \opDeliver{o_2}  \ar[r]_{\seqLinearp} & \opWrite{Memory[p].y,w} \ar@{--}[d]_{\id{consruct}} \\
\opread{x}{v} \ar[rrr]_{\seqLinearp} & & & \opwrite{y,w}
}
\]

 \begin{enumerate}
   \item $\PredPOB{L(K)}{}$ that delivers must follow their corresponding broadcasts in the local order.
 \end{enumerate}

\subheader{Case 3: write, write} 
Then $o_1=\opwrite{x,v}$ and $o_2=\opwrite{y,w}$

Two writes in program order are also ordered by message order, so their delivers and associated writes must also follow this order.

\begin{xy}
\xymatrix{
\opwrite{x, v} \ar[rr]^(0.3){\programOrder{}} & \ar@{=>}[d]  & \opwrite{y, w} & \\
\opBcast{[x, v, \widehat{p}, \_]} \ar[rr]^(0.3){\ProgramOrder{}} & \ar@{=>}[d]  & \opBcast{[y, w, \widehat{p}, \_]} & \\
\opDeliver{[x, v, \widehat{p}, \_]} \ar[rd]_{\ProgramOrder{}}  \ar[rr]^(0.3){\widehat{delorder}} & \ar@{=>}[d] & \opDeliver{[y, w, \widehat{p}, \_]} \ar[r]^{\ProgramOrder{}} & \opWrite{\id{Memory}[\widehat{q}].y, w} \\
& \opWrite{\id{Memory}[\widehat{q}].x, v} \ar[ru]_{\ProgramOrder{}} & & 
}
\end{xy}

\subheader{Case 4: write, read } 
 $o_1=\opwrite{x,v}$ and $o_2=\opread{y}{w}$

In both fast write and slow write algorithms there is a \func{WaitWritesComplete} call so that :

\[
\xymatrix{
\opBcast{[\const{write},x,v]} \ar[r]^{\ProgramOrder} \ar[d]_{\seqLinearp}   &  \func{WaitWritesComplete} \ar[rr]^{\ProgramOrder} & &  \opRead{y}{w}  \ar@{--}[dd]_{\id{construct}} \\
  \opDeliver{[\const{write},x,v]} \ar[r]_{\seqLinearp}   &  \opWrite{x,v} \ar@{|-->}[u]^{1.}_{\seqLinearp} \ar@{--}[d]_{\id{construct}} & \\
& \opwrite{x,v} \ar[rr]_{\seqlinearp} & & \opread{y}{w} 
}
\]

\begin{enumerate}
  \item Property of \func{WaitWritesComplete}. All previously broadcasted writes must be delivered before it completes.
\end{enumerate}

Thus in all cases we have $o_1 \orderArrow{L_p} o_2$.
Therefore $\orderArrow{L_p}$ extends $\orderArrow{\programOrder}$.

\end{specialproof}

Case 4 of the proof is an example of how we can simplify these types of proofs.  
The only property needed is that there is a \func{WaitWritesComplete} between the \opbcastVoid{} and the \opread{}.
Both \swimpl{}{}{} and \fwimpl{}{}{} satisfy this property and so we can prove the correctness of both implementations with one proof.
Also notice that we do not need to specify the specific \func{WaitWritesComplete} instance used; as long as there is at least one, the proof still holds.

\begin{lemma}
\label{top-middle-group-ordering}
  $\forall p,q\in P, i\in [1,k] :  \Pred{Agree}[ \orderArrow{L_p},  \orderArrow{L_q}, O|\cutwritesgroup{S_i} ]$
\end{lemma}

\begin{specialproof}
Let $W_1, W_2$ be write operations in some $O| \cutwritesgroup{S_i}$.
Then the broadcasts of these writes in the transformation are $\opBcast{msg_{w_1}} \in \wimpl{K}{L(K)}{W_1}$\\ and  $\opBcast{msg_{w_2}} \in \wimpl{K}{L(K)}{W_2}$.
Since they share the same group, we can observe that $\func{label}(msg_{w_1})=\func{label}(msg_{w_2})$.

For processes $p$ and $q$ there are target writes that are produced from the transformation of $W_1$ and $W_2$. 
Then let $w_{1p}, w_{1q}, w_{2p}, w_{2q} $ be these corresponding writes in $O_{\widehat{C}}$.
Suppose WLOG that $w_{1p} \relLinearp{} w_{2p}$, then 
$\opDeliver{ msg_{w_1} } \relLinearp{} w_{1p} \relLinearp{} \opDeliver{ msg_{w_2} } \relLinearp{} w_{2p} $ which implies 
$\opDeliver{ msg_{w_1} } \relLinearp[\widehat{q}]{} w_{1q} \relLinearp[\widehat{q}]{} \opDeliver{ msg_{w_2} } \relLinearp[\widehat{q}]{} w_{2q} $ since $\PredPOB{L(K)}{}$ requires that deliveries of messages with the same label must agree.
\end{specialproof}


\subsection{Correctness of \tokenimpl{L}{} transformation}

Let $\Processes$ be a multiprogram that uses \opreadVoid{}s, \opwriteVoid{}s, \opbcastVoid{}s, and for each process, only calls \opdeliverVoid{} from at most one thread, calls \opbcastVoid{} from at most one thread, and \opbcastVoid{} and \opdeliverVoid{} are never called by the same thread.

\begin{theorem}
  $\tokenimpl{L}{}$ correctly implements  \PredPOB{L}{} on \PredNW{},
for any $L$.
\end{theorem}

\begin{specialproof}

\specialsubheader{Assume:} 

Let $\widehat{C}$ be a computation in $\ComputationSet{\tokenimpl{L}{\Processes}, \PredNW{}}$ and let $C$ be an interpretation of $\widehat{C}$.

To show $\PredPOB{L}{C}$ we construct witness orders that satisfy the requirements of Definition \ref{general-pob-defn}.

\specialsubheader{Build:}


Choose some collection of witness orders $\MapSet{(O|\widehat{p}, \orderArrow{\seqLinearp}): \widehat{p} \in  \tokenimpl{L}{P}}$ to $\PredNW{\widehat{C}}$.

Recall that for a total order $(O,\orderArrow{X})$, its induced sequence is denoted by $X$.
For each $p$, construct the sequence $L_p$ as follows:

\begin{itemize}
\item Take the sequence $\widehat{L_{\widehat{p}}}$ formed from the witness total order $(\widehat{O}|\widehat{p}, \orderArrow{ \widehat{L_{\widehat{p}}}})$ to  $\PredNW{\widehat{C}}$ and form ${Short}(\seqLinearp)$ by removing:
  \begin{enumerate}
    \item all operations on the handshake variables $\id{need-token}_l$ and $\id{door}_l$ for all $l\in L$.
    \item all \opSendVoid{} and \opRecvVoid{} operations except: the first \opSendVoid{} of a  $\func{bcastop}()$ and the \opRecvVoid{} of a \opdeliverVoid{}.
  \end{enumerate}
  Note that each remaining operation was produced from the transformation of some specification level operation, rather than a thread created by the transformation.
\item Associate the target level operations in ${Short}(\seqLinearp)$ with specification level ones by defining $\constructArrow$ as follows: 

  For this proof we just have to associate these target level operations with the specification level operations that produced them.

  \begin{tabular}{|rl|c|}
    \hline
   Target Operation  in transformation & Let \\
    \hline
    $\opRead{x}{v} \in   \tokenimpl{L}{\opread{x}{v}}$ & $\opRead{x}{v}\constructArrow \opread{x}{v}$.  \\
   $\opWrite{x,v}  \in  \tokenimpl{L}{\opwrite{x,v}}$ & $\opWrite{x,v}\constructArrow \opwrite{x,v}$.  \\
   $\tokenimpl{L}{\opbcast{m,l}}._1\opSend{s,d,m}$   & $\opSend{s,d,m}\constructArrow \opbcast{s,d,m}$. \\ 
   $\opRecv{s,d,m}    \in \tokenimpl{L}{\opdeliver{m , l}}$ & $\opDequeue{queue}{m}\constructArrow \opdeliver{m , l}$.\\  
  \hline  
  \end{tabular}
\item Construct the sequence \seqlinearp{} from $Short(\seqLinearp)$ by replacing all the target level operations with their associated specification level operations .
\end{itemize}

Tokens strictly order events in time, the hard part of this proof is ensuring that the ordering provided to the tokens properly enforces orderings on the operations performed while the token is ordered.
While the concept behind the implementation is simple, the proof must use the specific ordering constraints provided by the target level model to prove correctness.
This exposes the parts of the proof that may need to be redone if for instance, the consistency of the shared variables between threads in the Network model is weakened.

\specialsubheader{Verify:}

The construction yields total orders $(O|p, \orderArrow{L_p})$ that are valid by the fact that projecting on to subsets of objects preserves validity of the variables.  The sequences of \opbcastVoid{} and \opdeliverVoid{} are valid since 1) the \opSendVoid{} of the \opbcastVoid{} \orderArrow{\HappensBefore{}} the \opDequeueVoid{} of its \opdeliverVoid{} and 2) each \const{ORD-MSG} is sent only once to each processor, received only once at each processor and enqueued only once at each processor.  


The following table shows the properties we prove to verify the constraints of Definition \ref{general-pob-defn}:

\begin{tabular}{|l| l | r |}
  \hline
  & Constraint & Lemma \\
  \hline
& $\forall p\in P: (O|p, \orderArrow{\seqlinearp} ) $ is a valid total order & By construction \\
& $\forall p\in P: \Pred{Extends}[O|p, \orderArrow{\seqlinearp{}}, \orderArrow{\programOrder{}}]$ & Lemma \ref{token-extend-program-lemma} \\
& $\forall p\in P: \Pred{Extends}[O|p, \orderArrow{\seqlinearp{}}, \orderArrow{delorder}]$ & Lemma \ref{token-fifo-lemma}  \\
& $\forall p, q\in P, l\in L: \Pred{Agree}[O|\cutdeliverslabel{l}, \orderArrow{\seqlinearp{}}, \orderArrow{\seqlinearp[q]{}}]$ & Lemma \ref{token-agree-lemma}  \\
  \hline
\end{tabular}\medskip


\end{specialproof}


\begin{lemma}
\label{token-extend-program-lemma}
 $\forall p\in P: \Pred{Extends}[O|p, \orderArrow{\seqlinearp{}}, \orderArrow{\programOrder{}}]$  \\
\end{lemma}

\begin{specialproof}

This proof is simplified because of the way transformations are defined, the memory model, and the choice of operations in the construction of the \orderArrow{\seqlinearp{}} orders.

Let $o_1, o_2 \in O|p$ such that $o_1 \orderArrow{\programOrder} o_2$. Let $\tsimpl{L}{o}.\opCommon{low}{o}{}$ be the operation in the transformation of $o$ so that $\tsimpl{L}{o}.\opCommon{low}{o}{} \constructArrow o$. 

\begin{xy}
\xymatrix{
o_1 \ar@{--}[d]_{\tokenimpl{L}{}} \ar[r]^{\programOrder{}} & o_2 \ar@{--}[d]^{\tokenimpl{L}{}}\\
\tokenimpl{L}{o_1} \ar[r]^{\ProgramOrder{}} & \tokenimpl{L}{o_2} \\
\tokenimpl{L}{o_1}.\opCommon{low}{o}{} \ar@{-(}[u] \ar[r]^{\ProgramOrder{}\cap\seqLinearp{}}_{1.} & \tokenimpl{L}{o_2}.\opCommon{low}{o}{} \ar@{-(}[u] \\
o_1 \ar@{--}[u]^{construct} \ar[r]^{\seqlinearp{}} & o_2 \ar@{--}[u]_{construct} \\
}
\end{xy}

\noindent 1. $\Pred{Extends}[O|\widehat{p}, \orderArrow{\seqLinearp}, \orderArrow{\ProgramOrder}]$
  
\end{specialproof}

The proofs in this paper often rely on preservation of program order to simplify proofs.  
Program order allows us to isolate subroutine calls and their effects in an effective way.

\begin{lemma}
\label{token-passtoken-total-order-lemma}
For all $l\in L$ let $T_{l} = \{\func{PassToken}_p() : \func{PassToken}_p()\subseteq O \}$.
then $(B_l, \orderArrow{\HappensBefore{}})$ is a total order.
\end{lemma}

\begin{specialproof}

  Either $$ \func{PassToken}^{1}(l) \orderArrow{\HappensBefore} \func{PassToken}^2(l) \textrm{ or }   \func{PassToken}^{2}(l) \orderArrow{\HappensBefore} \func{PassToken}^1(l) $$ since there is only one original \opSendVoid{} for each token at the beginning of $\func{TokenThread}_l$, and each $\func{PassToken}.\opRecvVoid{}$ has exactly one corresponding \opSendVoid{} which is either the original \opSendVoid{} or the \opSendVoid{} at the end of a \func{PassToken}. 

\end{specialproof}

\begin{lemma}
\label{token-handshake-lemma}
 Let $p\in P$, $n, d \in V$
 $T_p = \{ \func{ProtectedBcast}(n,d,m,l) :  \func{ProtectedBcast}(n,d,m,l) \subseteq{} O \}$ 
 and $ G_p = \{ \func{Guard}(n,d) : \func{Guard}(n,d) \subseteq{} O \} $
Then there exists an injection $\func{protected-by}: T_p \mapsto G_p $ so that:

\noindent
$\func{protected-by}\left(\func{ProtectedBcast}(n, d, m, l)\right) = \func{Guard}(n,d) $ 

if and only if
 
\noindent
$ \xymatrix{ \func{ProtectedBcast}(n, d, m, l).\func{bcastop} \ar@{|-->}[r]^{\HappensBefore{}} &  \func{Guard}(n, d) } $\\
and \\
$ \xymatrix{ \func{ProtectedBcast}(n, d, m, l).\func{bcastop} & \ar@{-->|}[l]_{\HappensBefore{}} \func{Guard}(n, d) } $ 
\end{lemma}

This lemma specifies the correctness of the handshake protocol in a way that it can be composed with the ordering provided by the token protocol.
Each \func{ProtectedBcast} ``inherits'' the ordering from a \func{Guard} and no two \func{ProtectedBcast} instances may share the same \func{Guard}.
The uniqueness condition requires us to properly ``reset'' the handshake variables when exiting a \func{Guard}.

\begin{specialproof}
  Let 
$$
  \begin{aligned}
    \func{protected-by}&(\func{ProtectedBcast}(n, d, m, l)) \defequal \\
    & \func{Guard}(n,d) : \func{Guard}(n,d).\opWrite{d, \mtrue{}} \orderArrow{\WritesInto} \func{ProtectedBcast}(n, d, m, l).\opRead{d}{\mtrue{}}
  \end{aligned}
  $$


Let $\id{PrB} = \func{ProtectedBcast}(n, d, m, l)$ and $G = \func{Guard}(n,d)$

  \begin{xy}
\xymatrix{
  G.\opWrite{d,\mtrue{}}\ar[r]_{\WritesInto} & \id{PrB}.\opRead{d}{\mtrue{}} \ar@{=>}[d] \ar[r]_{\ProgramOrder} & \id{PrB}.\func{bcastop} \\
  G \ar@{-->|}[rr]_{\HappensBefore} & & \id{PrB}.\func{bcastop}
}
  \end{xy}

Other:

\begin{xy}
\xymatrix{
    \func{ProtectedBlock}^1.\func{bcastop} \ar[r]^{\ProgramOrder} & \func{ProtectedBlock}^1.\opWrite{need, \mfalse{}} \ar[r]^{\WritesInto} \ar@{=>}[d] &   G.\opRead{need}{\mfalse{}} \\
    \func{ProtectedBlock}^1.\func{bcastop} \ar@{|-->}[rr]_{\HappensBefore{}} & & G
}
\end{xy}

We now show that $\func{ProtectedBlock}^1 = \id{PrB}$.

Since all the \func{ProtectedBlock} instances are called by the same thread they are totally ordered by program order.  There are 3 cases:

Case $ \func{ProtectedBlock}^1 = \id{PrB}$ : done.

Case $ \id{PrB} \orderArrow{\ProgramOrder} \func{ProtectedBlock}^1 $

\begin{xy}
\xymatrix{
\id{PrB}.\opWrite{need, \mfalse{}} \ar[r]^{\ProgramOrder{}}_{2.} & \func{ProtectedBlock}^1.\opRead{need}{\mtrue{}} \ar[r]^{\ProgramOrder{}} & \func{ProtectedBlock}^1.\opwrite{need, \mfalse{}} \ar[dd]^{\seqlinearp{}}_{1.}\\
\id{PrB}.\opRead{doorOpen}{\mtrue{}} \ar[u]^{\ProgramOrder{}} \\
G.\opWrite{doorOpen, \mtrue{}} \ar[u]^{\seqlinearp{}}_{1.} & & G.\opRead{need}{\mfalse{}} 
}
\end{xy}

\noindent
1. $G, \id{PrB}, $ and $\func{ProtectedBlock}^1$ were chosen to satisfy these properties.

\noindent
2. Since $\orderArrow{\seqlinearp}$ is valid, there must be a \opWrite{need,\mtrue{}} between the $G.\opWrite{need,\mtrue{}}$ and $G.\opRead{need}{\mfalse}$  but since all \func{Guard} calls on the same handshake variables are in the same thread, $G$ must perform this write, which is not possible by the code. Contradiction.

Case $ \func{ProtectedBlock}^1 \orderArrow{\ProgramOrder} \id{PrB}$

\begin{xy}
\xymatrix{
 \func{ProtectedBlock}^1.\opWrite{need, \mfalse{}} \ar[rr]^{\ProgramOrder{}} \ar[d]_{\WritesInto{}} & & \id{PrB}.\opRead{need}{\mtrue{}} \\
    G.\opRead{need}{\mfalse{}} \ar[urr]_{\seqLinearp{}}^{1.} & & G.\opWrite{need, \mtrue{}} \ar[u]_{\WritesInto{}} \\
}
\end{xy}

\noindent
1.  $G.\opWrite{need, \mtrue{}}$ must be ordered between these two operations in \orderArrow{\seqLinearp{}}, but then $G.\opWrite{need, \mtrue{}} \orderArrow{\ProgramOrder{}} G.\opRead{need}{\mfalse{}}$ and $G.\opRead{need}{\mfalse{}} \orderArrow{\seqLinearp{}} G.\opWrite{need, \mtrue{}}$.  Contradiction.

\func{protected-by} is injective since all the \func{Guard} instances are in the same thread and are totally ordered by program order.



\end{specialproof}

\begin{lemma}
For all $l\in L$, let $B_{l} = \{\tokenimpl{L}{\opbcast{u,l}}.\func{bcastop} : \opbcast{u,l} \in O\}$
then $(B_l , \orderArrow{\HappensBefore{}})$ is a total order.
\end{lemma}

\begin{specialproof}
Let $l\in L$, $\func{protected-by}$ be a function provided by Lemma \ref{token-handshake-lemma}.  

Let
 $b_1 = \tokenimpl{L}{\opbcast{u_1,l}}.\func{bcastop}$, $b_2 = \tokenimpl{L}{\opbcast{u_2,l}}.\func{bcastop}$ be distinct elements of $B_l$.

Then let $\func{PassToken}^{1}= \func{protected-by}(b_1)$ and $\func{PassToken}^{2}= \func{protected-by}(b_2)$.


By the Lemma \ref{token-passtoken-total-order-lemma}, the \func{PassToken} instances are totally ordered.
 Suppose WLOG that $ \func{PassToken}^{1} \orderArrow{\HappensBefore} \func{PassToken}^2$ then:

\begin{xy}
\xymatrix{
\func{PassToken}^{1} \ar[rr]_{\HappensBefore} \ar@{)-}[d] & & \func{PassToken}^2 \ar@{)-}[d]\\
\func{PassToken}^1.\func{Guard} \ar[rr]^{\HappensBefore}  & & \func{PassToken}^2.\func{Guard} \ar@{-->|}[d]^{\HappensBefore}_{1.}\\
b_1 \ar[rr]^{\HappensBefore}_(0.4){2.}  \ar@{|-->}[u]^{\HappensBefore}_{1.} &  & b_2  \\
}
\end{xy}

\begin{enumerate}
\item By Lemma \ref{token-handshake-lemma} and construction of $\func{PassToken}^1$ and $\func{PassToken}^2$. 
\item By 1 and the order on the \func{Guard} instances.
\end{enumerate}

\end{specialproof}

\begin{lemma}
\label{token-fifo-lemma}  
 $\forall p\in P: \Pred{Extends}[O|p, \orderArrow{\seqlinearp{}}, \orderArrow{delorder}]$  \\
\end{lemma}

\begin{specialproof}

  Let $o_1, o_2\in O|p$  such that $o_1 \orderArrow{delorder} o_2$.

  Then $o_1 = \opdeliver{u_1,l_1}, o_2 = \opdeliver{u_2,l_2}$ and
$\opbcast{u_1,l_2} \orderArrow{\programOrder} \opbcast{u_2, l_2}$.

  \begin{xy}
    \xymatrix{
      \opbcast{u_1, l_1} \ar[r]^{\programOrder} \ar@{--}[d]_{\func{TokenPOB}} & \opbcast{u_2, l_2} \ar@{--}[d]^{\func{TokenPOB}} \\
      \tokenimpl{L}{\opbcast{u_1, l_1}}.\opSend{s, p, m_1} \ar[r]^{\ProgramOrder} \ar[d]_{\MessageOrder} & \tokenimpl{L}{\opbcast{u_2,l_2}}.\opSend{s, p, m_2} \ar[d]^{\MessageOrder} \\
      \tokenimpl{L}{\opdeliver{u_1, l_1}}.\opRecv{s, p, m_1} \ar[r]_{\FifoChannel\cap\seqLinearp} & \tokenimpl{L}{\opdeliver{u_2, l_2}}.\opRecv{s, p, m_2} \\
      \opdeliver{u_1, l_1} \ar[r]_{\seqlinearp} \ar@{--}[u]^{construct} & \opdeliver{u_2, l_2} \ar@{--}[u]_{construct}
    }
  \end{xy}

\end{specialproof}


\begin{lemma}
\label{token-agree-lemma}
 $\forall p, q\in P, l\in L: \Pred{Agree}[O|\cutdeliverslabel{l}, \orderArrow{\seqlinearp{}}, \orderArrow{\seqlinearp[q]{}}]$  \\
\end{lemma}

\begin{specialproof}

Let $l\in L$ define a relation $ \orderArrow{label_l}$.

$\opdeliver{u_1, l}\orderArrow{label_l}\opdeliver{u_2,l} \defequal \tokenimpl{L}{\opbcast{u_1,l}}.\func{bcastop} \orderArrow{\ProgramOrder} \tokenimpl{L}{\opbcast{u_2,l}}.\func{bcastop}$

$(O|\cutdeliverslabel{l}, \orderArrow{label_l})$ is a total order.

 
Let \opdeliver{u_1,l} \orderArrow{label_l} \opdeliver{u_2,l} and $m_1, m_2$ be their respective matches, then $(m_1.ts, m_1.src) < (m_2.ts, m_2.src)$ and $m_1.ts \le m_2.ts$ so 

\begin{xy}
  \xymatrix{
 \tokenimpl{L}{\opbcast{u_1, l}}.\func{bcastop} \ar[r]^{\HappensBefore} & \tokenimpl{L}{\opbcast{u_2, l}}.\func{bcastop} \ar@{-->|}[d]^{\HappensBefore} \\
 \tokenimpl{L}{\opdeliver{u_1,l}} \ar[r]^{\HappensBefore} \ar@{|-->}[u]^{\HappensBefore} & \tokenimpl{L}{\opdeliver{u_2,l}}\\
 \tokenimpl{L}{\opdeliver{u_1,l}}.\opRecvVoid{} \ar@{-(}[u] \ar[r]^{\HappensBefore\cap\seqLinearp{}} & \tokenimpl{L}{\opdeliver{u_2,l}}.\opRecvVoid{} \ar@{-(}[u] \\
 \opdeliver{u_1,l} \ar[r]_{\seqlinearp{}} \ar@{--}[u]^{construct} & \opdeliver{u_2,l} \ar@{--}[u]_{construct}
}
\end{xy}

\end{specialproof}


\subsection{Correctness of the Timestamp implementation }

We illustrate these proof techniques by presenting (up to space constraints) the proof that the transformation 
\tsimpl{L}{P} correctly implements a multiprogram $P$ for the \POBName{} model, for any label set $L$,
on the \NWName\ model.
The proofs of correctness of the transformation from \PredPC{K}{} to \PredPOB{L(K)}{}
for each of the transformations \swimpl{}{}{} and \fwimpl{}{}{}, 
generalize the ideas of Attiya and Welch \cite{DBLP:journals/tocs/AttiyaW94} (corrected in \cite{attiya2004dcf}). 
They are in the full version of the paper \cite{cheng2009thesis}.


Let $\Processes$ be a multiprogram that uses \opreadVoid{}s, \opwriteVoid{}s, \opbcastVoid{}s, and for each process, only calls \opdeliverVoid{} from at most one thread.

\begin{theorem}
  $(\tsimpl{L}{P}, \PredNW{})$ implements $(P, \PredPOB{L}{})$ where $\opdeliverVoid{}$ is called from at most one thread in each process.
\end{theorem}

\begin{specialproof}
%We use the general outline of memory consistency proofs from Section \ref{proofs.structure.section}.

\specialsubheader{Assume:}
Let $\widehat{C}$ be a computation in $\ComputationSet{\tsimpl{L}{\Processes}, \PredNW{}}$ and let $C$ be an interpretation of $\widehat{C}$.

To show $\PredPOB{L}{C}$ we construct witness orders that satisfy the requirements of Definition \ref{general-pob-defn}.

\specialsubheader{Build:}
Choose some collection of witness orders $\MapSet{(O|\widehat{p}, \orderArrow{\seqLinearp}): \widehat{p} \in  \tsimpl{L}{P}}$ to $\PredNW{\widehat{C}}$.

Recall that for a total order $(O,\orderArrow{X})$, its induced sequence is denoted by $X$.
For each $p$, construct the sequence $L_p$ as follows:

\begin{itemize}
\item Take the sequence $\widehat{L_{\widehat{p}}}$ formed from the witness total order $(\widehat{O}|\widehat{p}, \orderArrow{ \widehat{L_{\widehat{p}}}})$ to  $\PredNW{\widehat{C}}$ and form ${Short}(\seqLinearp)$ by removing:
  \begin{enumerate}
  \item all the operations on the $\id{T}$, $\id{counter}$, and $\id{local-counter}$ variables.
  \item all \opSendVoid{} and \opRecvVoid{} operations except: the \opSendVoid{} of a  $[\const{local-broadcast-request}]$.
  \item all priority queue operations except \opDequeueVoid{} operations.
    \item all fifo queue operations except \opFIFODequeueVoid{} operations.
  \end{enumerate}
  Note that each remaining operation was produced from the transformation of some specification level operation, rather than a thread created by the transformation.
\item Associate the target level operations in ${Short}(\seqLinearp)$ with specification level ones by defining $\constructArrow$ as follows: 

  For this proof we just have to associate these target level operations with the specification level operations that produced them.

  \begin{tabular}{|rl|c|}
    \hline
   Target Operation & in transformation & Let \\
    \hline
    \opRead{x}{v}   & $\tsimpl{L}{\opread{x}{v}}$ & $\opRead{x}{v}\constructArrow \opread{x}{v}$.  \\
   \opWrite{x,v}   & $\tsimpl{L}{\opwrite{x,v}}$ & $\opWrite{x,v}\constructArrow \opwrite{x,v}$.  \\
   \opSend{s, d, [\const{L-B-R}]}  & $\tsimpl{L}{\opbcast{u, l}}$ & $\opSend{s, d, [\const{L-B-R}]}\constructArrow \opbcast{u, l}$. \\ 
   \opDequeue{queue}{m}  &  $\tsimpl{L}{\opdeliver{m.update , m.label}}$ & $\opDequeue{queue}{m}\constructArrow \opdeliver{m.update , m.label}$.\\  
   \opFIFODequeue{\id{fifo}[p]}{m} & $\tsimpl{L}{\opdeliver{m.update , m.label}}$ & $\opFIFODequeue{\id{fifo}[p]}{m}\constructArrow \opdeliver{m.update , m.label}$.\\
  \hline  
  \end{tabular}
\item Construct the sequence \seqlinearp{} from $Short(\seqLinearp)$ by replacing all the target level operations with their associated specification level operations .
\end{itemize}



\specialsubheader{Verify:}
The construction yields total orders $(O|p, \orderArrow{L_p})$ that are valid by the fact that projecting on to subsets of objects preserves validity of the variables.  The sequences of \opbcastVoid{} and \opdeliverVoid{} are valid since 1) the \opSendVoid{} of the \opbcastVoid{} \orderArrow{\HappensBefore{}} the \opDequeueVoid{} of its \opdeliverVoid{} and 2) each \const{ORD-MSG} is sent only once to each processor, received only once at each processor and enqueued only once at each processor.  
 The sequence $Short(\seqLinearp)$ is valid for all objects except queues, so by replacing the \opDequeueVoid{} operations with \opdeliverVoid{} operations, we regain validity.
The following table shows the properties we prove to verify the constraints of Definition \ref{general-pob-defn}:

\begin{tabular}{|l| l | r |}
  \hline
  & Constraint & Lemma \\
  \hline
& $\forall p\in P: (O|p, \orderArrow{\seqlinearp} ) $ is a valid total order & By construction \\
& $\forall p\in P: \Pred{Extends}[O|p, \orderArrow{\seqlinearp{}}, \orderArrow{\programOrder{}}]$ & Lemma \ref{timestamp-extend-program-lemma} \\
& $\forall p\in P: \Pred{Extends}[O|p, \orderArrow{\seqlinearp{}}, \orderArrow{delorder}]$ & Lemma \ref{timestamp-fifo-lemma} \\
& $\forall p, q\in P, l\in L: \Pred{Agree}[O|\cutdeliverslabel{l}, \orderArrow{\seqlinearp{}}, \orderArrow{\seqlinearp[q]{}}]$ & Lemma \ref{timestamp-agree-lemma} \\
  \hline
\end{tabular}\medskip

\end{specialproof}

The timestamp implementation enforces an agreement between processes on the order that updates are delivered in, rather than ordering them in time.
It does not rely on the target level constraints as directly as the token implementation, and most of the difficulty in this proof is in the ordering provided by the specific way that the implementation uses timestamps.
A key feature of this implementation is that it is optimized so that it can avoid sending acknowledgments in some cases.


%% Let $C$ and $\widehat{C}$ be computations such that \\ $\widehat{C}\in (\tsimpl{L}{\Processes}, \tsimpl{L}{J}, \PredNW{})$ and $\widehat{C} \modelArrow{\func{TS-POB}^{*-1}} C$. This matches the \specialsubheaderinline{Assume} step of Theorem \ref{tokenpob-correctness-theorem}.

%% Let $(M,\orderArrow{MO})$ and $\MapSet{ (O|p,\orderArrow{ { L_{{p}} } }) : {p}\in {P}:  }$ be constructed from the witness orders $\MapSet{ (O|\widehat{p},\orderArrow{ { \seqLinearp } }) : \widehat{p}\in {P}:  }$.  
%% This matches the \specialsubheaderinline{Build} step of  Theorem \ref{tokenpob-correctness-theorem}.



We prove the required lemmas: two key technical lemmas, \ref{timestamp-deliver-key-lemma} and \ref{timestamp-counter-onestep-lemma}, and three lemmas \ref{timestamp-extend-program-lemma}-\ref{timestamp-agree-lemma} that glue these results to the theorem.


\begin{lemma}
\label{timestamp-deliver-key-lemma}
If $\opSend{s_1,d_1,m_1}, \opSend{s_2,d_2,m_2} \in O$ so that $m_1.l \ne \bot$ and $m_2.l \ne \bot$
  $m_1.ts \le m_2.ts $ and $ \opDequeue{queue_h}{m_2} \in O|p $ then $ \opEnqueue{queue_g,m_1} \orderArrow{\ProgramOrder{}} \opDequeue{queue_h}{m_2}$

\end{lemma}
\begin{specialproof}

Let $m_1, m_2$ be \const{ORD-MSG} messages so that $\opSend{s_1, d_1, m_1}, \opSend{s_2, d_2, m_2} \in O$ and
  $m_1.ts \le m_2.ts $ and $ \opDequeue{queue_h}{m_2} \in O|p $.

By examining the transformation $\opDequeue{queue_h}{m_2}$ must come from the transformation of a $\opdeliver{u_2}$.
$m_1$ and $m_2$ have corresponding spec level updates $u_1$ and $u_2$, respectively.

Let $q = m_1.src$. 

Before $m_2$ was dequeued, we must have read a greater or equal timestamp from $T[q]$.
This must have been caused by some message $rm$ with this timestamp from $T[q]$.
This message $rm$ is either $m_1$ or must have been sent after $m_1$.  
We consider the case that $m_1 \ne rm$.

\[
\xymatrix{
\tsimpl{L}{\opdeliver{u_2}}.\opDequeueVoid{} & \\
\ar[u]_{\ProgramOrder} \tsimpl{L}{\opdeliver{u_2}}.\opRead{T[q]}{rts : rts \geq m_2.ts \geq m_1.ts} \\
   \ar[u]_{\ProgramOrder\cap \orderArrow{\seqLinearp{}}}^{1.} \func{HandleMessage}^1().\opWrite{T[q],rts} & \\ 
   \func{HandleMessage}^1().\opRecv{\widehat{q},\widehat{p},rm: rm.ts = rts}  \ar[u]_{\ProgramOrder} & \opSend{\widehat{q},\widehat{p},rm} \ar[l]_{\MessageOrder}     \\
 & \ar@{=>}[l]\\
  \ar[uu]^{\FifoChannel}  \opRecv{\widehat{q}, \widehat{p}, m_1} &    \ar[uu]_{\ProgramOrder} \ar[l]_{\MessageOrder} \opSend{\widehat{q},\widehat{p}, m_1}   \\
}
\]

\noindent
1. By the validity \seqLinearp{} there must be a \opWriteVoid{} that wrote that value.  Since \opDeliverVoid{} is only in one thread, \func{HandleMessage} instances can only be in that thread, so they must be ordered in program order.

By examining the code, we can see that the \opRecvVoid{} of $m_1$ must have been followed by an \opEnqueueVoid{}, and since the \opRecvVoid{}s are executed by a single thread, this must have happened before \opRecv{rm}. Isolating an area of the previous diagram and adding in the \opEnqueueVoid{} gives:

\[
\xymatrix{
\tsimpl{L}{\opdeliver{u_2}}.\opDequeueVoid{} & \\
 \ar[u]^{\ProgramOrder} \opRecv{rm}  &  & &  \ar[lll]^{\FifoChannel} \ar[lld]^{\ProgramOrder}_{1.} \opRecv{m_1}\\
          &   \ar[ul]^{\ProgramOrder}_{2.} \opEnqueue{m_1} &     &\\
}
\]

\noindent
1. $m_1$ is a \const{ORD-MSG}. The \func{HandleMessage} instance that received $m_1$ will \opEnqueueVoid{} it. \\
2. The \opRecvVoid{} operations must come from separate \func{HandleMessage} instances, which must be by the same thread.

Therefore $  \opEnqueue{m_1} \orderArrow{\ProgramOrder} \tsimpl{L}{\opdeliver{u_2}}.\opDequeue{queue_i}{m_2}$.

\end{specialproof}

Lemma \ref{timestamp-deliver-key-lemma} is the essential safety property of the broadcast algorithm. 
A process can only dequeue a message when it is sure that it has ``seen'' and enqueued all messages that might have a smaller timestamp.


\begin{lemma}
\label{timestamp-counter-onestep-lemma}
If  $m_2$ is \const{ORD-MSG} sent by some $q\in P$ with $m_2.counter \ge 2$  then there is a \const{ORD-MSG} $m_1$ sent by the same $q$ such that $m_1.counter = m_2.counter -1$. \\
 If $d_1 = \opDequeue{queue_h}{m_2}$ or $\opFIFODequeue{\id{fifo}[q]}{m_2}$ $d_2 \in O|p$ for some $p \in P$ then $d_1 \orderArrow{\ProgramOrder} d_2$ for some $d_1 = \opDequeue{queue_i}{m_1}$ or $\opFIFODequeue{\id{fifo}[q]}{m_1}$. 
\end{lemma}
\begin{specialproof}
$m_1$ must exist since the counter is incremented to a value $c$ exactly when an \const{ORD-MSG} is created with that counter value $c$. 

To deliver $m_2$ we must have $\opread{counter[src]}{m_2.counter - 1}$.
We can see from the code that $counter[src]$ starts at $0$ and can only be incremented by 1 each time a message from that source is delivered.
This means that $counter[src]$ consecutively gets the value of each element in $[1,m_2.counter-1]$ at some point before $\opread{counter[src]}{m_2.counter - 1}$.
So, we must have delivered $m_1$ before $m_2$, as this diagram illustrates:

\[
\xymatrix{
\opDequeue{queue_g}{m_2}  \ar@{-(}[r] & \tsimpl{L}{\opdeliver{m_2.update , m_2.label}}  \\
& \ar[lu]_{\ProgramOrder\cap\seqLinearp{}}^{1.} \opRead{counter[src]}{m_2.counter - 1 }  \ar@{-(}[u] \\
 & \ar[u]_{\seqLinearp{}}^{2.} \opWrite{counter[src], m_2.counter -1}  \ar@{-(}[d] \\
 \ar[ur]_{\ProgramOrder\cap\seqLinearp{}}^{3.} \opDequeue{queue_h}{n:n.counter = m.counter - 1}   \ar@{-(}[r] & \tsimpl{L}{\opdeliver{n.update, n.label}}\\
}
\]

\begin{enumerate}
\item Examine the definition of $\tsimpl{L}{\opdeliver{m , l}}$. The \func{CanDeliver} call before a \opDequeueVoid{} invocation must return \const{true}.
\item If the read value is greater than the initial value of 0, the value must have been written by a previous deliver call.  This deliver is $\opdeliver{n.update,n.label}$ for some message $n$.
\item Examine the definition of $\tsimpl{L}{\opdeliver{n.update,n.label}}$ the only write to counter occurs right after a dequeue.
\end{enumerate}

$n=m_1$ since different $\const{ORD-MSG}$ messages from the same process have distinct counter values. 
\end{specialproof}

\begin{corollary}
\label{timestamp-counter-deliver-lemma}
If $m_1, m_2$ are \const{ORD-MSG} messages and $\widehat{p} = m_1.src = m_2.src$ and $m_1.counter < m_2.counter$ then if $d_2 = \opDequeue{queue_h}{m_2}$ or $ \opFIFODequeue{\id{fifo}[\widehat{p}]}{m_2} $ and $d_2 \in O|p$ implies $d_1 \orderArrow{\ProgramOrder} \opDequeue{queue_h}{m_2}$ for some $d_1 = \opDequeue{queue_g}{m_1}$ or $\opFIFODequeue{\id{fifo}[\widehat{p}]}{m_1}$. 
\end{corollary}
\begin{specialproof}

Since $m_1.counter < m_2.counter$, the counter of $m_1$ must be in the set $[1,m_2.counter -1 ]$. 
Also observe that $m_1.counter >0$ so $m_1.counter \geq 1$ and $m_2.counter \geq 2$.

Apply Lemma \ref{timestamp-counter-onestep-lemma} result inductively to get:
\[
d_1 \orderArrow{\ProgramOrder} d_2 
\]

Where 
$d_1 = \opDequeue{queue_g}{m_1}$ or $\opFIFODequeue{\id{fifo}[\widehat{p}]}{m_1}$
and
$d_2 = \opDequeue{queue_h}{m_2}$ or $\opFIFODequeue{\id{fifo}[\widehat{p}]}{m_2}$.

\end{specialproof}


\begin{lemma}
\label{timestamp-extend-program-lemma}
 $\forall p\in P: \Pred{Extends}[O|p, \orderArrow{\seqlinearp{}}, \orderArrow{\programOrder{}}]$  \\
\end{lemma}

\begin{specialproof}
This proof is simplified by of the way transformations are defined, the memory model, and the choice of operations in the construction of the \orderArrow{\seqlinearp{}} orders.

Let $o_1, o_2 \in O|p$ such that $o_1 \orderArrow{\programOrder} o_2$. Let $\tokenimpl{L}{o}.\opCommon{low}{o}{}$ be the operation in the transformation of $o$ so that $\tokenimpl{L}{o}.\opCommon{low}{o}{} \constructArrow o$. 

\begin{xy}
\xymatrix{
o_1 \ar@{--}[d]_{\tsimpl{L}{}} \ar[r]^{\programOrder{}} & o_2 \ar@{--}[d]^{\tsimpl{L}{}}\\
\tsimpl{L}{o_1} \ar[r]^{\ProgramOrder{}} & \tsimpl{L}{o_2} \\
\tsimpl{L}{o_1}.\opCommon{low}{o}{} \ar@{-(}[u] \ar[r]^{\ProgramOrder{}\cap\seqLinearp{}}_{1.} & \tsimpl{L}{o_2}.\opCommon{low}{o}{} \ar@{-(}[u] \\
o_1 \ar@{--}[u]^{construct} \ar[r]^{\seqlinearp{}} & o_2 \ar@{--}[u]_{construct} \\
}
\end{xy}

\noindent 1. $\Pred{Extends}[O|\widehat{p}, \orderArrow{\seqLinearp}, \orderArrow{\ProgramOrder}]$
  
\end{specialproof}

\begin{lemma}
\label{timestamp-fifo-lemma}  
 $\forall p\in P: \Pred{Extends}[O|p, \orderArrow{\seqlinearp{}}, \orderArrow{delorder}]$  \\
\end{lemma}
\begin{specialproof}
  Let $o_1, o_2\in O|p$  such that $o_1 \orderArrow{delorder} o_2$.

  Then $o_1 = \opdeliver{u_1,l_1}, o_2 = \opdeliver{u_2,l_2}$ and
$\opbcast{u_1,l_2} \orderArrow{\programOrder} \opbcast{u_2, l_2}$.

  \begin{xy}
    \xymatrix{
      \tsimpl{L}{\opbcast{u_1, l_1}}.\opSendVoid{} \ar[r]^{\ProgramOrder} \ar[d]_{\MessageOrder} & \tsimpl{L}{\opbcast{u_2,l_2}}.\opSendVoid{} \ar[d]^{\MessageOrder} \\
      \func{HandleMessage}^1.\opRecvVoid{} \ar[r]^{\FifoChannel{}} \ar[d]_{\ProgramOrder} &    \func{HandleMessage}^2.\opRecvVoid{} \ar[d]_{\ProgramOrder}  \\
      \func{HandleMessage}^1.\opWrite{\id{local-counter},x} \ar[d]_{\ProgramOrder} \ar[ur]_{\ProgramOrder} & \func{HandleMessage}^2.\opWrite{\id{local-counter},y} \ar[d]_{\ProgramOrder}\\
      \func{HandleMessage}^1.\opSend{m_1} & \func{HandleMessage}^2.\opSend{m_2}  
      }
  \end{xy}

Since the \id{local-counter} monotonically increases,  $0< m_1.counter = x < y = m_2.counter$.

By Corollary \ref{timestamp-counter-deliver-lemma} we have $ \opDequeue{queue_g}{m_1} \orderArrow{\ProgramOrder{}}  \opDequeue{queue_h}{m_2}$ thus:

\begin{xy}
  \xymatrix{
    \opDequeue{queue_g}{m_1} \ar[r]^{\ProgramOrder{}\cap\seqLinearp{}}_{1.} & \opDequeue{queue_h}{m_2} \\
     \opdeliver{u_1, l_1}  \ar@{--}[u]^{construct} \ar[r]_{\seqlinearp{}} & \opdeliver{u_2, l_2} \ar@{--}[u]^{construct}
  }
\end{xy}

\noindent 1. $\Pred{Extends}[O|\widehat{p}, \orderArrow{\seqLinearp}, \orderArrow{\ProgramOrder}]$

As required.

\end{specialproof}


\begin{lemma}
\label{timestamp-agree-lemma}
 $\forall p, q\in P, l\in L: \Pred{Agree}[O|\cutdeliverslabel{l}, \orderArrow{\seqlinearp{}}, \orderArrow{\seqlinearp[q]{}}]$  \\
\end{lemma}

\begin{specialproof}

Define $\func{match}(\opdeliver{u, l}) = m : \tsimpl{L}{\opdeliver{u,l}}.\opDequeue{queue_g}{m}$.

  Let $l\in L$, define a total order $(O|\cutdeliverslabel{l}, \orderArrow{\id{label}_l})$.
 
\[\opdeliver{u_1,l} \orderArrow{\id{label}_l} \opdeliver{u_2,l} \defequal (m_1.ts, m_1.src) < (m_2.ts, m_2.src) \]

where $m_1 = \func{match}(\opdeliver{u_1, l})$, $m_2 = \func{match}(\opdeliver{u_2, l})$ and $<$ compares pairs lexicographically.
 
We now show that every \orderArrow{\seqlinearp{}} agrees with \orderArrow{\id{label}_l}.

Let \opdeliver{u_1,l} \orderArrow{\id{label}_l} \opdeliver{u_2,l} and $m_1, m_2$ be their respective matches, then $(m_1.ts, m_1.src) < (m_2.ts, m_2.src)$ and $m_1.ts \le m_2.ts$ so 
by Lemma \ref{timestamp-deliver-key-lemma}: 

\begin{xy}
  \xymatrix{
    \opEnqueue{queue_l, m_1} \ar[rr]^{\ProgramOrder{}} \ar[dr]_{\ProgramOrder{}} & \ar@{=>}[d]^{1.} & \opDequeue{queue_l}{m_2} \\
    & \opDequeue{queue_l}{m_1} \ar[ru]^{\ProgramOrder\cap\seqLinearp{}}_{2.} & \\
    & \opdeliver{u_1, l}  \ar@{--}[u]^{construct} \ar[r]_{\seqlinearp{}} & \opdeliver{u_2, l} \ar@{--}[uu]^{construct}
  }
\end{xy}

\begin{enumerate}
\item Since the priority queue is ordered by lexicographic $<$ on $(m.ts, m.src)$.  
\item $\Pred{Extends}[O|\widehat{p}, \orderArrow{\seqLinearp}, \orderArrow{\ProgramOrder}]$
\end{enumerate}

\end{specialproof}



